Experimental validation of an explicit flatness-based MPC design for quadcopter position tracking

Due to the nonlinearities and operational constraints typical to quadcopter missions, Model Predictive Control (MPC) encounters the major challenge of high computational power necessary for the online implementation. This problem may prove impractical, especially for a hardware-limited or small-scale setup. By removing the need for online solvers while keeping the constraint satisfaction and optimality, Explicit MPC (ExMPC) stands out as a strong candidate for this application. Yet, the formulation was usually hindered by the two main problems: nonlinearity and dimensionality. In this paper, we propose an ExMPC solution for the quadcopter position stabilization by analyzing its description (dynamics and constraints) in the flat output space. With the former issue, the system is exactly linearized into a concatenation of three double integrators at a price of cumbersome constraints in the new coordinates. For the latter, with a suitable characterization of these constraints, the stabilizing ExMPC can be computed for each double integrator separately. The controller is then validated via simulations and experimental tests. The proposed scheme achieves similar performance and guarantees to the state-of-the-art solution but with notably less computational effort, allowing scalability in a centralized manner

==> texfiles/intro_v1.tex <==
%Start with MPC+FL
Naturally separated into translational and rotational dynamics, the navigation of multi-rotors is typically divided into the correspondingly two hierarchical layers of control: position and attitude control \cite{nascimento2019position}. 
In such a setup, the position control (outer) loop computes the necessary thrust 
and rotation to generate the vehicle's vertical, longitudinal and lateral motion to follow a reference, 
while the attitude controller (inner loop) is responsible for achieving those required configurations from the outer loop at a higher bandwidth.
In this work, we focus on the position control problem with a view to navigating the vehicle while respecting
its operating constraints and ensuring stability.

Although being investigated for decades \cite{wang2021efficient,greeff2022fly,Torrente9361343}, optimally governing these thrust-propelled vehicles remains an interesting topic in the research community due to their trigonometric nonlinearity and challenges to provide a constraint satisfaction guarantee.
One increasingly popular approach employs Model Predictive Control (MPC) where a constrained optimization problem is solved to compute the optimal input action over a finite horizon in the future \cite{nguyen2019stabilizing,nguyen2020stability,Luis8950150,nan2022nonlinear}.
However, 
it is well known that 
the strategy requires high computational power and relatively long sampling time due to the model's nonlinearity.
% when the nonlinear model is used to predict the system's motion, the strategy will require relatively high computational power to find the optimal control online.
% This burden not only makes the in-flight computation time undesirably long, but also proves challenging to construct stability proof in the control synthesis.
Facing the issue, as an intrinsic characteristic of the vehicle,
the properties of differentially flat systems has been exploited 
as a bridge between nonlinear system analysis and linear control theory.
More specifically, with the fact that all the states and inputs of a differentially flat system can be expressed in terms of 
the flat output, and a finite number of its derivatives, the theory paves different paths to remedy the system nonlinearity, especially in optimization-based solutions.

On one hand, thanks to the differential parameterization via the flat output, a solution to the system's differential equation can be generated via curve fitting approaches for both input and state vectors. Then, along such a trajectory, Taylor series can be exploited to approximate the dynamics into a linear time varying system which is then efficiently handled by scheduling the MPC \cite{prodan2013receding,nguyen2017multi,Cohen9143426}. 
While the MPC problem is simplified to a Quadratic Program (QP), one major theoretical drawback for this approach resides on how to quantify the model's approximation error and analyze the stability for the original nonlinear system, especially in non-trivially high dimension.
On the other hand, with the input-output relationship provided by the flat representation, the vehicle is guaranteed to be dynamic feedback linearizable, i.e., the system can be equivalently represented by integrator chains \cite{levine2009analysis} in a new coordinate system, called the flat output space. Therefore, by linearizing the dynamics in closed-loop, the previously mentioned drawback is sidestepped.
Nevertheless, with this direction, a critical difficulty rises from the complicated input constraints during the conversion between the original space and the flat output space.
% Particular results \cite{nguyen2018effective,mueller2013model,thinhECC23,freire2023flatness}
% quadcopters' constraints on thrust, attitude and angular rate are mapped into high order derivatives of the flat output
Particular results on sketching theses new constraints for quadcopters from thrust, attitude and angular rate can be found in \cite{nguyen2018effective,mueller2013model,freire2023flatness}, which map the original physical limits to nonlinear sets of the flat output and up to third order derivatives. 
In \cite{thinhECC23,mueller2013model,greeff2018flatness}, linear approximation of these constraints was employed in an MPC setting, which reduces the complexity of the navigation and preserves the system's
stability analysis in a linear representation. 

With the goal of advancing toward a low-cost solution while maintaining both constraint and stability guarantees, explicit MPC (ExMPC) formulation constitutes a promising candidate \cite{bemporad2002explicit}. The underlying idea is to convert nonlinear control of the quadcopter's position control into a standard QP problem via flatness, with a stability guarantee via common axioms in MPC \cite{mayne2000constrained} and finally solve such problem within the  multi-parametric quadratic programming framework \cite{takacs2016python}.
The online implementation includes 
locating the current state inside the solutions computed offline as a set of critical regions, and evaluating the corresponding optimal control action associated to such a region.
Although there exists related works in the literature \cite{jiajin2017design,liu2015explicit}, the discussed methods appear to rely on
a near hovering approximated model or lack stability quantitative arguments. 
Furthermore, to the best of the authors' knowledge, although the simulation findings in these works affirms the theory, the effectiveness of the strategy has not been experimentally validated for the model under study.
Therefore, 
exploiting the exactly linearized model in closed-loop of the quadcopter's translational dynamics, we:
\begin{itemize}
    \item introduce a synthesis procedure for implementing the ExMPC to the outer loop of the quadcopter via its exact linearization from flatness with a linear description for the convoluted constraints. 
    \item analyze the dimensionality challenges as well as the computational advantages via simulation tests, and validate the method via an experimental nano-drone platform. The experiment video is available at \urlvideo.
\end{itemize}

While the flat representation was already well discussed in the literature \cite{thinhECC23}, we focus on the implementation of the ExMPC controller
and its ancillary technical prospects. More specifically, in Section \ref{sec:rep}, the quadcopter position control problem in both the state/input state and the flat output space will be recalled. Section \ref{sec:formulation} presents the procedure to formulate 
the QP problem, which is then later solved
with multi-parametric QP tools. Therein, simulations are also provided to analyze the applicability of the strategy and to compare the advantage with the implicit MPC law. Section \ref{sec:validation} verified the position control scheme via various experimental tests. Finally, conclusion and future directions are discussed in Section \ref{sec:conclusion}.

\textit{Notation:} Matrices with appropriate dimension are denoted via bold upper-case letters. Bold lower-case letter represents vectors. $\|\bx\|_{\boldsymbol{P}}\triangleq\sqrt{\bx^\top \boldsymbol{P} \bx}$ denotes the weighted norm. The letter $k$ represents the signal's value at the discrete step $kt_s$ with the sampling time $t_s$.  $\mathrm{ls}(n, a, b)$ represents a set of $n$ evenly spaced real numbers over the  interval $[a,b]$. $\ominus$ denotes the Pontryagin difference. $\mathrm{conv}\{\cdot\}$ denotes the convex hull of given components.
